AniTrack: A Power-Efficient, Time-Slotted and Robust UWB Localization System for Animal Tracking in a Controlled Setting

Accurate localization is essential for a wide range of applications, including asset tracking, smart agriculture, and animal monitoring. While traditional localization methods, such as Global Navigation Satellite System (GNSS), Wi-Fi, and Bluetooth Low Energy (BLE), offer varying levels of accuracy and coverage, they have drawbacks regarding power consumption, infrastructure requirements, and deployment flexibility. Ultra-Wideband (UWB) is emerging as an alternative, offering centimeter-level accuracy and energy efficiency, especially suitable for medium to large field monitoring with capabilities to work indoors and outdoors. However, existing UWB localization systems require infrastructure with mains power to supply the anchors, which impedes their scalability and ease of deployment. This underscores the need for a fully battery-powered and energy-efficient localization system. This paper presents an energy-optimized, battery-operated UWB localization system that leverages Long Range Wide Area Network (LoRaWAN) for data transmission to a server backend. By employing single-sided two-way ranging (SS-TWR) in a time-slotted localization approach, the power consumption both on the anchor and the tag is reduced, while maintaining high accuracy. With a low average power consumption of 20.44 mW per anchor and 7.19 mW per tag, the system allows fully battery-powered operation for up to 25 days, achieving average accuracy of 13.96 cm with self-localizing anchors on a 600 m2 testing ground. To validate its effectiveness and ease of installation in a challenging application scenario, ten anchors and two tags were successfully deployed in a tropical zoological biome where they could be used to track Aldabra Giant Tortoises (Aldabrachelys gigantea).

==> content/05_field_deployment.tex <==


% IMPORTANT %
% THIS SECTON IS MOVED TO SYSTEM CHARACTERIZATION %



\section{Field Deployment}\label{field_application}
To evaluate the proposed system, including the data collection backend, the outlined setup is tested in a real-world deployment by tracking Aldabra Giant Tortoises in a zoological environment in collaboration with the Zoo Zurich. %Studying the movement of these animals is particularly interesting, as it may provide insights into their social interactions within a group, preferred locations within their habitat, and activity patterns over time. Such insights can help zookeepers to continuously improve animal welfare.  

This application was chosen because high accuracy is required to determine the precise location of each tortoise and its proximity to others. To gain further insights into the tortoise's behavior and the environmental situation, additional sensors have been used, as described in \cref{system_overview}, providing data on temperature, humidity, and orientation.  

The system was installed with a localization period of \qty{40}{\second}, acquiring data for a two-hour period.  

To ensure a flexible localization setup, the anchors are mounted on \qty{1.5}{\meter} wooden poles, as shown in \cref{fig:final_setup}, which can be easily mounted without additional installation requirements. Additionally, two tags are attached to the tortoises’ carapaces using double-sided silicon tape, allowing for easy removal without leaving residue.  

The final setup installed on the animals is illustrated in \cref{fig:final_setup}, while \cref{fig:tortoise_path_monitoring} presents a selection of the collected position data of a tortoise. The monitored enclosure covers a total area of approximately \qty{126}{\square\meter}.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/torotoise.png}
    \caption{Real-world evaluation, monitoring the location of Aldabra Giant Tortoises in the \textsc{Zoo Zürich}.}
    \label{fig:final_setup}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/tortoise_path_monitoring.png}
    \caption{The movement path of one tortoise within its enclosure, demonstrating how the setup can be applied for monitoring animal behavior and social interaction.}
    \label{fig:tortoise_path_monitoring}
\end{figure}
